PCFGaze: Physics-Consistent Feature for Appearance-based Gaze Estimation

Although recent deep learning based gaze estimation approaches have achieved much improvement, we still know little about how gaze features are connected to the physics of gaze. In this paper, we try to answer this question by analyzing the gaze feature manifold. Our analysis revealed the insight that the geodesic distance between gaze features is consistent with the gaze differences between samples. According to this finding, we construct the Physics- Consistent Feature (PCF) in an analytical way, which connects gaze feature to the physical definition of gaze. We further propose the PCFGaze framework that directly optimizes gaze feature space by the guidance of PCF. Experimental results demonstrate that the proposed framework alleviates the overfitting problem and significantly improves cross-domain gaze estimation accuracy without extra training data. The insight of gaze feature has the potential to benefit other regression tasks with physical meanings.

==> figures/CtnLoss.tex <==
\begin{figure}
\begin{center}
% \begin{overpic} 
% [width=\linewidth]
% {example-image-a}
% \end{overpic}
\includegraphics[width=\linewidth]{figures/assets/CtnLoss.pdf}
\end{center}
% \vspace{-2mm}
\caption{
Continuity Loss of the baseline model in the test set. The Continuity Loss is close to 0 when the gaze differences between samples are below 20\degree and raise quickly when gaze differences are larger.
}
\label{fig:CtnLoss}
% \vspace{-2mm}
\vspace{2mm}
\end{figure}

==> figures/Iso_ori.tex <==
\begin{figure}
\begin{center}
% \begin{overpic} 
% [width=\linewidth]
% {example-image-a}
% \end{overpic}
\includegraphics[width=\linewidth]{figures/assets/Iso_ori.pdf}
\end{center}
% \vspace{-2mm}
\caption{
The results of Isomap. 512 dimensional gaze features are mapped into 3 dimensional space. Data points distribute on the surface of a sphere approximately, which is similar to the unit sphere of gaze direction vectors.
}
\label{fig:IsoOri}
% \vspace{-2mm}
\vspace{2mm}
\end{figure}

==> figures/Outlier.tex <==
\begin{figure}
\begin{center}
% \begin{overpic} 
% [width=\linewidth]
% {example-image-a}
% \end{overpic}
\includegraphics[width=\linewidth]{figures/assets/Outlier.pdf}
\end{center}
% \vspace{-2mm}
\caption{
Gaze estimation errors for abnormal samples in ETH-XGaze: (a) closed eyes, (b) dark image, (c) wrong annotation and (d) occluded eyes. Gaze label is visualized as red arrows. Intuitively, they should result in failure cases. However, estimation errors of Baseline method are small (within 1 time std. range) due to overfitting. In contrast, \pa~produces significantly larger errors, which correspond with the abnormal input. 
}
\label{fig:Outlier}
% \vspace{-2mm}
\vspace{2mm}
\end{figure}

==> tables/BaseAccuracy.tex <==
\begin{table*}
\caption{
% 
Cross-domain gaze estimation results in degree. The proposed \proposed~method achieves improvements as large as $29.23\%$ without any extra training data.Percentage in red indicates largest improvement. The results of \prp~are shown in row 5. $^*$ mean that the number of neighbors in geodesic distance is customized for each source domain (100, 800 and 300 for \ETH, \GazeC~and \MPII~respectively). For fairness, We only take results in row 5 for comparison.
% 
} % \caption
\renewcommand\arraystretch{1.1} %1.1
\centering
\resizebox{\linewidth}{!}{ %< auto-adjusts font size to fill line
\begin{tabular}{@{}cl|cc|cc|ccc@{}}

\toprule[1.3pt]
&Method &    \ETH $\rightarrow$\MPII  &  \ETH $\rightarrow$\ED   &  \GazeC$\rightarrow$\MPII   &  \GazeC$\rightarrow$\ED   &  \MPII $\rightarrow$\ETH &  \MPII $\rightarrow$\GazeC   &  \MPII $\rightarrow$\ED  \\
% \hline
\midrule[0.6pt]
1&Baseline \cite{cheng2022puregaze} &  8.13  &  7.74  &  9.89  &   11.42 & -   & -   & -   \\

2&PureGaze \cite{cheng2022puregaze}    &  \marka{7.08} \upscore{12.92}  &  7.48 \upscore{3.36}   &  9.28 \upscorered{6.17}  &  \marka{9.32} \upscorered{18.39}  &  -  &  -  &  -   \\
\midrule[0.6pt] \midrule[0.6pt]
% \hline \hline
3&Baseline    &  8.64  &  7.83   &  8.68  &  12.35  &  14.03  &  15.48  &  16.15  \\ 

4&Baseline+\pa  &  7.92 &  8.22   &  8.33  &  11.40  &  14.14  &  14.83  &  11.80  \\ %neighbor:300

5&\prp   &  7.40 \upscorered{14.35} &  \marka{7.30} \upscorered{6.77} &  \marka{8.36} \upscore{3.69}  &  10.18 \upscore{17.57}  &  \marka{13.69} \upscorered{2.42}  & \marka{ 13.76} \upscorered{11.11}  &  \marka{12.40} \upscorered{23.22}  \\ %neighbor:300
% \hline
\midrule[0.6pt]

%   & \multicolumn{2}{c|}{\prp~with 100 neighbors} & \multicolumn{2}{c|}{\prp~with 800 neighbors} & \multicolumn{3}{c|}{\prp~with 300 neighbors}\\
% & \multicolumn{7}{l|}{\prp~with 100, 800, 300 neighbors for \ETH, \GazeC and \MPII~respectively}\\
6&Baseline+\pa$^*$  &  7.98 &  8.45   &  7.79  &  10.97  &  14.14  &  14.83  &  11.80  \\ %neighbor:300

7&\prp$^*$   &  7.00 \upscore{18.98} &  7.02 \upscore{10.34} &  7.71 \upscore{11.18}  &  8.74 \upscore{29.23}  &  13.69 \upscore{2.42}  &  13.76 \upscore{11.11}  &  12.40 \upscore{23.22}  \\

\bottomrule[1.3pt]
\end{tabular}
} %< \resizebox

\label{tab:BaseAccuracy}
\end{table*}

% baseline+\prp &  22.68 (0.31)  &  7.4 (1.24) &  7.3 (0.53)  &  20.87 (-1.73) &  8.36 (0.32)  &  10.18 (2.17)  &  13.69 (0.34)  &  13.76 (1.72)  &  11.67 (4.48)  \\ %neighbor:300
% PureGaze \cite{cheng2022puregaze}  & -   &  7.08 (1.05)  &  7.48 (0.26)  & -  &  9.28 (0.61)  &  9.32 (2.1)  &  -  &  -  &  -   \\
% Baseline+\pa~800 &  23.62  &  7.19  &  7.32  & 19.3  &  7.76  &  10.97  & 14.15   &  14.37  &  11.98  \\
% baseline+\prp~800 &  22.91  &  7.36  &  7.4  &  21.16 &  7.71  &  8.74  &  12.66  &  14.46  &   13.44 \\
% Baseline+\pa~100 &  25.88  &  7.98  &  8.45  & 18.67  &  8.28  &  13.34  &  14.04  &  14.83  &  12.99  \\
% baseline+\prp~100 &  22.76  &   7.00 &  7.02  &  19.33 &  8.63  &  15.28  &  14.74  &  14.49  &  12.02  \\
